A Semi Black-Box Adversarial Bit-Flip Attack with Limited DNN Model Information

Despite the rising prevalence of deep neural networks (DNNs) in cyber-physical systems, their vulnerability to adversarial bit-flip attacks (BFAs) is a noteworthy concern. This paper proposes B3FA, a semi-black-box BFA-based parameter attack on DNNs, assuming the adversary has limited knowledge about the model. We consider practical scenarios often feature a more restricted threat model for real-world systems, contrasting with the typical BFA models that presuppose the adversary's full access to a network's inputs and parameters. The introduced bit-flip approach utilizes a magnitude-based ranking method and a statistical re-construction technique to identify the vulnerable bits. We demonstrate the effectiveness of B3FA on several DNN models in a semi-black-box setting. For example, B3FA could drop the accuracy of a MobileNetV2 from 69.84% to 9% with only 20 bit-flips in a real-world setting.

==> backup.tex <==
\subsection{Model Extraction}
Because neural network models are confidential information, it is impossible to have direct access to them. Therefore model extraction is an emerging field that tries to steal the model.
Most of the existing model extractions were developed for adversarial attacks around two main objectives: output similarity of extracted model and the actual model on the same input(fidelity) and accuracy[High Accuracy and High Fidelity Extraction of Neural Networks]. Because the objective of adversarial attacks is to make an input that misleads the model to a wrong output, fidelity, and accuracy, which only rely on input and output, have proven practical. However in bit flip attack we need the exact value and position of each weight. Meaning that even with a fidelity of 100\% the attack will perform similar to a random attack since we do not know the exact value and position of each weight. Therefore among various model extractions techniques that were developed on adversarial attack, we focus on those which give us the exact value and position of each bit.


\subsubsection{Architecture Extraction}
A side-channel attack is one of the existing model extractions that takes advantage of hardware-based exploitation\cite{naghibijouybari2018rendered}–\cite{chowdhuryy2020branchspec}. These attacks can be used to leak sensitive information about the model, such as architecture\cite{yan2020cache}–\cite{hu2020deepsniffer}, \cite{zhang2021stealing}–\cite{duddu2018stealing}. Model structure can be extracted through microarchitecture attacks \cite{yan2020cache}, physical side channels\cite{batina2018csi}, and bus snooping attacks\cite{hu2020deepsniffer} with very high accuracy. Although most of the existing side-channel attacks can infer high-level model information, such as model architectures, they are not successfully stealing complete information about model parameters (weight bits).


\subsubsection{Parameter Extraction}
In \cite{rakin2021deepsteal}, they propose an advanced model extraction attack framework that effectively steals DNN weights with the aid of a memory side-channel attack. They used the rowhammer-based hardware fault technique as the information leakage vector. This attack is the expanded version of rambled\cite{kwong2020rambleed}, revealing that the rowhammer fault characteristic can be leveraged to leak victim information. Although Deepsteal can extract detailed model parameters, the extraction is only partial, and they are capable of extracting up to 90\% of all weight bits.






\subsection{Data importance} [[should be removed?]]
Previous bitflip-attacks assume having access to a batch of the test datasets(bitflip-attack). However, this assumption is not practical as they want to avoid it in other fields such as quantization(zeroq). Two of the previous works in bit-flip attacks(bdfa and zebra) also mentioned this constraint and solved it. The data attributes, such as privacy and real-time, play an essential role. For example, in self-driving cars, the data is collected in real-time with sensors and can not be replicated easily, or personal health records and encrypted data, which are hard to obtain because of privacy issues.



\subsection{Vulnerability ranking of DNN Parameters}
In \cite{rakin2019bit} and all the following works of Parameter Attacks, finding the vulnerable bits is an essential part of attack since attacking random bits in the model barely affect the accuracy, even after 100 bit-flips (less than 1\% accuracy drop). Thus, an importance estimation of each parameter (or parameter bits) is needed to measure the importance of a parameter for the functionality and output of the model. If a parameter has a higher importance value, it is more vulnerable and sensitive to perturbation, thus attacking them will crush the DNN more efficiently.

The importance estimation in Deep Learning models has been explored through different avenues. Many metrics has been proposed from DNN pruning and quantization methods, Adversarial input attacks, etc, that can be counted as a vulnerability estimation. These estimations can be divided into two parts: data dependant methods and the data independent ones. 


\subsubsection{Data Dependent Importance Estimation} 
There are a group of importance estimations that use the gradient or hessian of the parameter to compute its importance. In \cite{goodfellow2014explaining} the gradient of a pixel was used to compute its importance and sensitivity to change. In \cite{molchanov2019importance} the importance of each weight was estimated by the first and second order of its Taylor expansion. Since this group of importance estimation needs to calculate the gradient (or Hessian matrix) for the weights, they need to compute the loss function, which needs both data and a full functional model.

\subsubsection{Data Free Importance Estimation} 
[[What is the State of Neural Network Pruning?]]
A very popular importance estimation method is to score parameters based on their absolute values. Some pruning methods compare scores locally, such as a fraction of the parameters with the lowest scores within each structural subcomponent of the network (e.g., layers or filters) \cite{han2015learning}. Others consider scores globally, comparing scores to one another irrespective of the part of the network in which the parameter resides \cite{lee2018snip},\cite{frankle2018lottery} [[What is the State of Neural Network Pruning?]]
These methods do not need any data nor a fully functional model to be computed and therefore can be usefull for a black-box setting vulnerability estimation.

==> test.tex <==


% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------
% -------------------------------------------------------------


\section{Experimental Setup} \label{sec:setup}
\subsection{DNN Architectures and Datasets}
We test B3FA on three widely used DNN models: ?, VGG16 and ResNet50. All of them are trained on two deep learning datasets, CIFAR-10 and CIFAR-100. Both CIFAR-10 and CIFAR-100 contain 60000 RGB images with a size of 32 * 32. We use the layer-wise symmetric uniform post quantization to quantize the DNN parameters. Each weight parameter is quantized into 8-bit singed integers in two's-complement format. All experiments are performed on an Intel ? GHz processor with 16 GB memory and an NVIDIA GeForce RTX 3060 Ti GPU.


To validate the efficacy of our approach, we compute the Top-1 and Top-5 classification accuracy. The baseline Top-1 and Top-5 accuracy values for DNN models trained on both datasets is shown in table ?.

\begin{table}[tb!]
\begin{center}
\vspace{0.1in}
% \caption{Runtime and memory space overheads (O/H) when deploying resilient DNN with \Toolname~in the inference stage.}
\vspace{-0.05in}    
\scalebox{1.0}{
\begin{tabular}
{|l|r|r|r|r|r|r|}
    \hline 

     &  \multicolumn{2}{|c|}{CIFAR-10}  & \multicolumn{2}{|c|}{ImageNet} & \multicolumn{2}{|c|}{CIFAR-100} \\   \cline{2-7}
     &Top1&Top5&Top1&Top5&Top1&Top5  \\   \hline 
    %  \multirow{4}{*}{\rotatebox{90}{CIFAR-10}} & 100\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\  
    \cline{1-7}  VGG16 & 0 & 0 & 0 & 0 & 0 & 0 \\  
    \cline{1-7} ResNet50 & 0 & 0 & 0 & 0 & 0 & 0  \\ 
    \cline{1-7} MobileNetV2 & 0 & 0 & 0 & 0 & 0 & 0   \\
    \hline
    
\end{tabular}
}
%\vspace{-0.05in}
    \label{tab:baseline}
\end{center}
\end{table}

\subsection{Attack Assumptions and simulation}
In our experiments, we assume having full access to the network’s architecture. However, unlike the previous works, we do not assume having any input data, no weight gradients, and only partially recovered weight bits. There is also no access to training algorithm nor any training hyper parameters. The recovery process of weight bits are simulated using the Bernoulli distribution for each bit. We define the Recovery Percentage ($RP$ ? ) as the probability of a bit getting extracted from the memory. Therefore in our simulations, a bit will be considered recovered with the probability of $RP$, or not recovered with the probability of $1-RP$. We use the Monte Carlo simulation settings to cover the range of possible outcomes. We simulate the recovery 10 times for each DNN to observe the performance of the attack on different recovered bits. The simulation process is done using PyTorch Framework.


\section{Experimental Results}


\subsection{results on different models and datasets}
% imagenet CIFAR-10 100 tamame modela
% jadvale gonde

\begin{figure*}[!ht]
	\begin{center}
		\vspace{-0.33in}
		\includegraphics[scale=0.34]{figs/Figure_1.png}
		\vspace{-0.1in}
		\caption{Model Accuracy after each iteration of B3Fa with several Recovery Rates on ResNet50, VGG16 and MobileNetV2, trained on different datasets. We run ten experiments for each model, and the region in shadow indicates the error-band.}
		\label{fig:aveAcc}
		\vspace{-0.3in}
	\end{center}	
\end{figure*}

Figure 4: B3Fa results on three datasets and two different architectures with several Recovery Rates. We run ten experiments and the region in shadow indicates the error-band.

We test B3FA on multiple datasets and multiple DNNarchitectures to evaluate its efficiency of finding vulnerable bits and destroying the model's functionality. We evaluate our approach with different Recovery Rates to observe the impact of NZR on the attack performance with less recovered models.

In the converging section, 40\% recovery was a good measure because it was the last point that B3FA selects almost the most significant numbers. From that point to 0\%, the NZR is not successfully estimating large numbers. Therefore in this section, we use a recovery rate higher than 40\% and increase it by 20\% each time until 80\%.

As discussed in the bit flip attack[], We can perform a limited amount of bit flips. Therefore We show the results in the range of 0 to 30 bit-flips.

\subsubsection{CIFAR-100}
The first row of figure ? shows the performance of B3FA on the CIFAR-100 dataset. The accuracy of ResNet50 drops to lower than 40\%, half of the base accuracy, with only 17,23, and 28 bit-flips for 80\% to 40\% recovery. We repeated the same experiment for vgg, and we can get to lower than 20\% with only 10,15, and 27 bit flips. With 80\% recovery, B3FA achieves the random accuracy with only 25 bit-flips.
\subsubsection{CIFAR-10}
The second row of figure 1 is for the CIFAR-10 dataset. With 80\% recovery, B3FA gets to less than 25\% with 10 and 30 bit-flips on the ResNet50 and vgg16 datasets. By reducing the recovery rate to 60\%, we get 25\% and 29\% accuracy on the ResNet50 and vgg16 datasets.
\subsubsection{ImageNet}
The third row of figure 1 is for the imagenet dataset. With 80\% recovery, B3FA gets to less than 25\% with 10 and 30 bit-flips on the ResNet50 and vgg16 datasets. By reducing the recovery rate to 60\%, we get 25\% and 29\% accuracy on the ResNet50 and vgg16 datasets.

\begin{figure}[!tb]
	\begin{center}
	    %\vspace{-0.1in}
		\includegraphics[width = 0.5\textwidth]{figs/gradcam1.pdf}
		\vspace{-0.3in}
		\label{fig:scaled-distrib-filter}
		\caption{The visualization of 3 different pictures before and after performing B3FA on ResNet50 architecture trained on ImageNet (using grad cam[]).}
		\vspace{-0.1in}
	\end{center}	
\vspace{-0.1in}
\end{figure}

\textbf{effect of B3FA on input data}. To have a better understanding of how B3FA manipulate the model output, we used a visualization technique called Grad-cam[]. Grad-cam highlights the important regions in the image. Figure 7 illustrates that B3FA changes the model concentration from the desired subject to nonrelevant objects. Thus, the model output an incorrect label.

\subsection{Results on various quantization bit-width}


\begin{table}[tb!]
\begin{center}
\vspace{0.1in}
% \caption{Runtime and memory space overheads (O/H) when deploying resilient DNN with \Toolname~in the inference stage.}
\vspace{-0.05in}    
\scalebox{1.0}{
\begin{tabular}
{|c|l|r|r|r|r|r|r|r|r|r|}
    \hline 

    \multicolumn{2}{|c|}{} &  \multicolumn{3}{|c|}{8-bit}  & \multicolumn{3}{|c|}{6-bit} & \multicolumn{3}{|c|}{4-bit} \\   \cline{3-11}
    \multicolumn{2}{|c|}{} &10&20&30&10&20&30&10&20&30  \\   \hline \hline
     \multirow{4}{*}{\rotatebox{90}{CIFAR-10}} & 100\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\  
    \cline{2-11} & 80\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 \\  
    \cline{2-11} &60\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0  \\
    \cline{2-11} & 40\% & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0 & 0   \\
    \hline
    
\end{tabular}
}
%\vspace{-0.05in}
    \label{tab:overhead}
\end{center}
\vspace{-0.4in}
\end{table}

To show the the performance of B3FA on different quantization bit-widths, we evaluate our approch on 8-bit, 6-bit and 4-bit quantized VGG16 trained on CIFAR-100. Table ? shows the 


\subsection{Study of different Reconstruction Methods}
In our experiments, we need to reconstruct the bits that are not recovered from memory. We call this step the \textit{Reconstruction} step. In this section, we compare different Reconstruction methods and see whether NZR has the best performance or not. We use All-Zeros (all the unrecovered bits will be assigned to zero) and All-Ones (all the unrecovered bits will be assigned to one) to compare with NZR. As shown in Table ? NZR is more accurate than the other methods since it combines the two other methods to fit well for the twos-complement format of parameters.

\begin{table}[tb!]
\begin{center}
\caption{The Accuracy of different reconstruction methods on different Reconstruction Percentages evaluated on VGG16 trained on ImageNet.}
\scalebox{0.90}{
\begin{tabular}{|l|c|c|c|c|c|}
\hline
    % \multicolumn{1}{|c|}{}& \multicolumn{3}{c|}{Recovery Percentage}\\
    \multicolumn{1}{|c|}{}& RP = 80\% &RP = 70\% & RP = 60\% &RP = 50\% & RP = 40\%\\
\hline
    All-Zeros & 80\%& 80\%& 80\%& 80\%& 80\%\\
    All-Ones & 50\%& 80\%& 80\%& 80\%& 80\% \\
    NZR (ours) & \textbf{60\%}& \textbf{60\%}& \textbf{60\%} & \textbf{60\%} & \textbf{60\%}\\
\hline    
\end{tabular}
}
\end{center}
\end{table}

\subsection{Comparison to other methods}
In this section, we compare the performance of our approach to find the most vulnerable bits against previous methods. Fig ? shows the results of attacking a VGG16 model trained on CIFAR-10, using BFA[], DBFA[], and B3FA (ours). Since we want to compare the performance of the vulnerable bit search for these methods, we use the same method to reconstruct the partially recovered models. particularly we use NZR which has the most accurate prediction as shown in the section 3.?.For BFA, we also assume we have access to a batch of input data.

In the fully recovered case (RP = 100\%), the performance of the other two methods is almost as same as B3FA, meaning that B3FA is still a considerable option in a white or semi-white box settings.

Since both BFA[] and DBFA[] are not black box attacks, they fail to destroy the DNN in the partially recovered settings (RP = 80\%, 60\%, 40\%). In the recovery rates of 80\%, 60\%, and 40\%, BFA and DBFA can only cause an accuracy drop of at most ?\% and ?\% respectively, after 100 bit-flips. However, B3FA is able to cause an accuracy drop of around ?\% in the same recovery rates, only after ? bit-flips. It shows that those methods are not usable for the black box setup, and they need to inject a lot more bit-flips to decrease the accuracy of the model. This is because the reconstructed model is not functional; After the reconstruction, the model's accuracy goes around 10.14\%, which is significantly lower than an ideal reconstructed model with 93.06\% classification accuracy. Therefore, the gradients of parameters with respect to the loss function are not accurate as they were with an ideal model.


\subsection{Vulnerable bit searching RunTime}
Table ? compares the runtime of B3FA with the white-box Bit-Flip attack[] on VGG16 trained on CIFAR-10. Since B3FA does not need any input or gradients, there would be no forward or backward propagation. Therefore B3FA's speed of searching for the vulnerable bits is much faster than other methods. Most of the computations in B3FA happen in the preprocessing step before the first iteration. We need to compute the l2-norm of each filter and sort them afterward. The time complexity of the preprocess would be $O(N_W \times log(N_F))$, where $N_W$ refers to the number of weights, and $N_F$ refers to the number of filters in the DNN model. The only negligible computation in each iteration is choosing the maximum filter and recomputing the l2-norm of that filter after the bit-flip. Therefore, the time complexity of each iteration would be $O(N_{bf} \times N_{W_{F^*}})$, where $N_{bf}$ is the number of iterations in which we pick the most vulnerable bits, and $N_{W_{F^*}}$ is the number of weights in the most vulnerable filter, in order to compute the l2-norm again.

\subsection{Evaluation of vulnerability estimation}
Here, we compare our vulnerability estimation to the previous gradient-based method [,]. We show that the selected vulnerable bits also have high scores using other methods, particularly gradient-based estimation. Fig ? shows the corresponding gradient to the bit selected in each iteration. It depicts that the selected parameters have a much bigger gradient value than the average gradient value of all the weights in the network. Also as shown in Fig ? b) the sign of the gradients are almost always the negative of the sign of the parameter. This means that each bit-flip in the selected vulnerable bits is along its gradient ascending direction w.r.t the loss of DNN. This will make the loss function to get bigger with huge steps, and thus make the accuracy drop.


\subsection{converge}
% We also compare our approach with random bit-flip attacks. Fig ? illustrates the results
This section shows that selecting the filter with the highest l2norm  is a good measure. Figure x shows B3FA performance with different recovery rates on the cifar-100 dataset. Based on this figure, by increasing the recovery rate, the performance of B3FA becomes better. Meaning that we could get to a random state with fewer bit flips. Note that 0\% recovery is equivalent to randomly selecting bits, and a 100\% recovery is a white box attack like the bit flip attack[]. 

Figure1: The convergence of B3FA on CIFAR-100 dataset after 100 bit flips compared to random flipping and white box.







% \subsection{Resilience Results} \label{sec:resilience-results}

% To demonstrate the efficacy of \Toolname, we compare the model resilience under different fault rates, between our \Toolname, state-of-the-art studies Clip-Act \cite{hoang2020ft} and Ranger \cite{chen2020ranger} that use a layer-wise globally bounded ReLU activation function to improve model resilience,
% %(\zf{provides more details about Ranger and confirms the one for Clip-Act}), 
% as well as unprotected DNNs. 


% Figure~\ref{fig:distvgg} compares the model accuracy distribution between different approaches under different fault rates, using the VGG16 network on CIFAR-10 dataset as a case study. The accuracy of the unprotected DNN model has a huge drop to around 10\% under fault injection, which clearly calls for resilience enhancement. In general, as the fault rate increases, the accuracy of the three protected DNNs decreases, because the protection becomes less effective and faults are more likely to be injected in critical bits, having a more substantial impact on the output classification. As shown in Figure~\ref{fig:distvgg},  \Toolname~can keep the accuracy within an acceptable range even at a high fault rate of $10^{-5}$, whereas Clip-Act \cite{hoang2020ft} and Ranger \cite{chen2020ranger} experience a significant accuracy drop at fault rates higher than $10^{-6}$ and $10^{-7}$, respectively.

% Figure~\ref{fig:aveAcc} compares the average accuracy between \Toolname, Clip-Act \cite{hoang2020ft}, Ranger \cite{chen2020ranger} and unprotected model under different fault rates, for various DNN architectures and datasets. 
% First, all three protection methods boost the accuracy under fault compared to the unprotected one, and \Toolname~achieves the best accuracy (i.e., resilience) among all.
% Second, compared to Clip-Act \cite{hoang2020ft}, when the fault rate becomes $3\times10^{-6}$ or higher, \Toolname~achieves a significantly higher accuracy. For example, at the fault rate of $3\times10^{-6}$, \Toolname~can still achieve a high accuracy of 84.81\% and 90.28\% for ResNet50 and VGG16 models on CIFAR-10 dataset, while Clip-Act can only achieve an accuracy of 52.47\% and 61.63\%. 
% Third, Ranger \cite{chen2020ranger} performs much worse than Clip-Act \cite{hoang2020ft} and \Toolname, even at a low fault rate of $10^{-7}$. At a higher fault rate than $10^{-7}$, Ranger is no longer effective in the protection against faults.
% This is because Ranger truncates an output faulty value to a big positive bound, which still propagates in the network.

% % Figure~\ref{fig:aveAcc} compares the average accuracy between \Toolname, Clip-Act \cite{hoang2020ft}, Ranger \cite{chen2020ranger} and unprotected model under different fault rates, for various DNN architectures and datasets. 
% % First, all three protection methods boost the accuracy under fault compared to the unprotected one, and \Toolname~achieves the highest accuracy among all.
% % Second, compared to Clip-Act \cite{hoang2020ft}, when the fault rate becomes $3*10^{-6}$ or higher, \Toolname~achieves a significantly higher accuracy. For example, at the fault rate of $3*10^{-6}$, \Toolname~can still achieve a high accuracy of \zf{Fix these numbers: xxx and xxx} for ResNet50 and VGG16 models on CIFAR-10 dataset, while Clip-Act can only achieve an accuracy of \zf{Fix these numbers: xxx and xxx}. 
% % Third, Ranger \cite{chen2020ranger} performs much worse than Clip-Act \cite{hoang2020ft} and \Toolname, even at a low fault rate of $10^{-7}$. At a higher fault rate than $10^{-7}$, Ranger is no longer effective in the protection against faults.


% % provides significant higher accuracy compared the two other similar approaches. 


% % As it can be seen, all protection methods boost accuracy compared with the unprotected one. Furthermore, the proposed \Toolname~provides significant more accuracy compared the two other similar approaches. 
% % For example, for a defect rate of $10^-5$ (3×$10^-6$) in the case of VGG16, \Toolname~accuracy is $78.75\%$ ($90.28\%$), whereas Clip-Act accuracy is $19.09\%$ ($61.63\%$), indicating a $59.66\%$ ($28.65\%$) gain in accuracy. Similar patterns can also be seen in the case of other networks, as shown in Figure \ref{fig:aveAcc}.
% % As it can be seen, all protection methods boost accuracy compared with the unprotected one. Furthermore, the proposed \Toolname~provides significant more accuracy compared the two other similar approaches. 
% % For example, for a defect rate of $10^-5$ (3×$10^-6$) in the case of VGG16, \Toolname~accuracy is $74.4\%$ ($*$), whereas Clip-Act accuracy is $17.9\%$ ($*$), indicating a $56.8\%$ ($28.8\%$) gain in accuracy. Similar patterns can also be seen in the case of other networks, as shown in Figure \ref{fig:aveAcc}. 

% \begin{figure}[!tb]
% 	\begin{center}
% 	    \vspace{-0.1in}
%  		\includegraphics[width=0.5\textwidth]{pdffigs/DisAccC10L.pdf}
%  	\vspace{-0.2in}
% 	\caption{Model accuracy distribution for \Toolname, Clip-Act \cite{hoang2020ft}, Ranger \cite{chen2020ranger} and unprotected DNN,
% 	using the VGG16 network on CIFAR-10 dataset, under different fault rates.}
% 	\vspace{-0.3 in}
% 	\label{fig:distvgg}
% 	\end{center}	
% \end{figure}



% \begin{figure*}[!ht]
% 	\begin{center}
% 		    \vspace{-0.33in}
% 		\includegraphics[scale=0.34]{pdffigs/RobustnessCompareL.pdf}
% 		\vspace{-0.1in}
% 		\caption{Average model accuracy for \Toolname, Clip-Act \cite{hoang2020ft}, Ranger \cite{chen2020ranger} and 
% 		unprotected DNN models, including ResNet50, VGG16, and AlexNet models on CIFAR-10 and CAFIR-100 datasets, under different fault rates.}
% 		\label{fig:aveAcc}
% 		\vspace{-0.3in}
% 	\end{center}	
% \end{figure*}

% \subsection{Time and Memory Space Overhead}

% \subsubsection{Training Step}
% %               ResNet  vgg AlexNet
% % training      340 ,    60      and 17
% % posttrain    21,       4,       and  1
% % overhead   6.2%,   6.7%   and 5.9%
% Since \Toolname~separates the conventional training for accuracy and post-training for resilience, it can maintain a small computational overhead. For example, 
% %Compared to traditional activation function, the locally adaptive activation function-based DNN has additional parameters to adjust in post train step. Thus, we explore the additional computational cost required in post-training step.
% the whole process of post-training for ResNet50, VGG16 and AlexNet models on CIFAR-10 dataset take about 21, 4 and 1 minutes, respectively. Considering the long runtime for conventional training of these models (340, 60, and 17 minutes), \Toolname~only adds around 5.9\% to 6.7\% extra runtime overhead.

% \begin{table}[tb!]
% \begin{center}
% \vspace{0.1in}
% \caption{Runtime and memory space overheads (O/H) when deploying resilient DNN with \Toolname~in the inference stage.}
% \vspace{-0.05in}    
% \scalebox{0.96}{
% \begin{tabular}
% {|c|l|r|r|r|r|r|r|}
%     \hline 

%     \multicolumn{2}{|c|}{} &  \multicolumn{3}{|c|}{Runtime (ms)}  & \multicolumn{3}{|c|}{Memory (Mb)} \\   \cline{3-8}
%     \multicolumn{2}{|c|}{} & ReLU & \Toolname & O/H  & ReLU & \Toolname & O/H\rule{0pt}{10pt} \\   \hline \hline
%     \multirow{3}{*}{\rotatebox{90}{CIFAR-10}} & ResNet50 & 9.820&10.869&10.68\% & 156.69 & 165.05 & 5.34\%\rule{0pt}{10pt}\\  
%     \cline{2-8}  & VGG16 & 5.324&5.600&5.18\% & 29.60 & 30.46 & 2.91\%\rule{0pt}{10pt}\\  
%     \cline{2-8}  & AlexNet & 3.037&3.175&4.54\% & 23.53 & 23.68 & 0.64\%\rule{0pt}{10pt}  \\
%     \hline
%     \multirow{3}{*}{\rotatebox[origin=c]{90}{CIFAR-100}} & ResNet50 & 9.877&10.974&11.11\% & 156.70 & 165.10 & 5.36\%\rule{0pt}{11pt}
%     \\  \cline{2-8}  & VGG16 & 5.178&5.487&5.97\% & 29.65 & 30.47 & 2.77\%\rule{0pt}{11pt}
%      \\  \cline{2-8}  & AlexNet & 3.001 & 3.224 & 7.43 \% & 23.53 & 23.69 & 0.68\%\rule{0pt}{11.5pt} \\
%     \hline
    
% \end{tabular}
% }
% %\vspace{-0.05in}
%     \label{tab:overhead}
% \end{center}
% \vspace{-0.4in}
% \end{table}

% \subsubsection{Inference Step}
% % Since an activation function is applied to the outputs of most DNN neurons, it will mainly contribute to the overall DNN inference time and memory usage footprint.
% % The proposed \Toolname~adds an extra computation to the inference step with FitReLU which lead to memory and runtime overheads via inference step.

% Compared to the original ReLU, FitReLU (Equation~\ref{eq:TNBRELU}) costs more computation and needs extra memory space to store the bound values $\lambda_1$ to $\lambda_N$.
% Table~\ref{tab:overhead} presents the time and memory space overheads of \Toolname~for various models and datasets in the inference step. Since most of the computations and memory storage happen in the convolutional and fully connected layers, the overheads introduced by \Toolname~is manageable. Shown in Table~\ref{tab:overhead}, the runtime overheads are less than 12\% and the memory space overheads are less than 6\%.


%  \begin{figure}[!h]
%  	\begin{center}
%  	    %\vspace{-0.1in}
%  		\includegraphics[width = 0.5\textwidth]{figs/table.pdf}
%  		\vspace{-0.15in}
%  		\caption{our quantization technique works by taking the common factor $\Delta$ from the entire network and deleting it. in this way we do not have the overhead of $X_{q}$. $\times$ $\Delta$}
%  		\vspace{-0.1in}
%  		\label{fig:DNN}
%  	\end{center}	
%  \vspace{-0.1in}
%  \end{figure}
 




% \section{Approach}
% This section proposes a novel attack to maliciously cause a Convolutional Neural Network system malfunction by flipping extremely small amounts of vulnerable weight bits. This attack only needs access to the network architecture and partial weights information. First, it reconstructs the non-extracted weight bits using the proposed Near Zero Reconstruction (NZR) method. NZR tries to estimate the non-extracted weight bits and make each parameter close to zero. Then for finding vulnerable weights, we propose filter-wise L2-norm ranking (FL2R). FL2R ranks every filter with respect to their L2-norm and tries to find the most sensitive parameter to crush these filters.

% \subsection{Problem Definition}
% Given DNN architecture and partially extracted weight bits of the model, we want to fully reconstruct the partially extracted weight bits. Then we aim to find the most vulnerable weights in the model. We flip the most significant bit of the vulnerable weights chosen among DNN parameters, their sign bit. The sign bit is the most sensitive in each parameter since it causes the most change in the parameter value. After a few bit-flips, the accuracy of the model will drastically decrease.

% All the weights in the given DNN are quantized to signed integers using symmetric uniform 4-bit quantization and contain 32 levels. The computing system normally stores the signed integer in two’s complement representation, owing to its efficiency in arithmetic operations (e.g.,mul). We define Wql as the quantized weights in layer L and Bql as the weight bits in layer L in the twos-complement format. We define BBL as the recovered information of DNN parameters using RAMBLEED. The value of X corresponds to the non-recovered bits. WNL and BNL correspond to the weights and weight bits after the Near Zero Reconstruction (NZR). The goal of NZR is to reconstruct BNL (WNL) as close as possible (in terms of Hamming distance) to The ideal weight bits BQL. Then the reconstructed weights WNL will be given to FL2R to find the most vulnerable parameters. FL2R firstly estimates the importance of each filter weight on the functionality of the DNN model. After ranking the filter weights by their importance estimation, FL2R finds the most vulnerable parameter in the filter and attacks its most significant bit. In other words, we try to disrupt the filter's functionality so that the output feature map gets deactivated in the proper moments and maybe gets activated during unwanted moments. This will make the desired final output of the network less accurate, thus causing an accuracy drop.

% \subsection{Quantization and Encoding}
% quantization and twos-complement representation:
% Since the conventional quantized DNNs use the twos complement format to store the parameters in the memory, we focus on this representation format. Suppose Wlfp is the floating-point weights of layer L and Wlq as their corresponding quantized signed integer (twos-complement) representation. We also denote Wlfpdq as the floating-point de-quantized weights in layer l. The symmetric uniform 4-bit quantizer transform the Wlfp to Wlq using the equations below:


% ∆wl = max(Wfpl )/(2Nq −1 − 1); Wfp l ∈ Rd (2)

% Wlq = round(Wfpl /∆wl)

% Wlfpdq = Wlq  · ∆wl (3)
 
% Where the step size (∆wl) will be computed and then used to calculate the Wlq. Given one weight element w ∈ Wl, the conversion from its binary representation (b = [bNq −1, ..., b0] ∈ {0, 1}Nq ) 
% in two’s complement can be expressed as: 

% w/∆w = g(b) = −2Nq −1 · bNq −1 + Nq −2 ∑ i=0 2i · bi (4)

% With the conversion relation described by g(·) in Eq. (4), we can inversely obtain the binary representation of weights B from its 
% fixed-point counterpart as well. Figure 2 illustrates several 4-bit signed integers in the twos-complement format. As can be seen, the Most Significant Bit (3rd bit) is zero for the positive integers and one for the negative integers. 0000 (0) is the smallest positive integer, and 0111 (7) is the biggest. Among the negative integers, 1000 (-8)* and  1111 (-1) are the smallest and biggest. 

% \subsection{Near Zero Reconstruction (NZR)}
% Since DNN weight bits are partially extracted, we need to reconstruct non-extracted bits in the best and accurate way possible. The distributions of weights and activations of pre-trained DNNs are bell-shaped such as Gaussian or Laplacian [17,35] (Fig?). That is, most of the weights are clustered around zero while few of them are spread in a long tail. It indicates that the probability of the value of a random weight being close to zero is much higher than having a higher absolute value. Therefore, NZR tries to reconstruct each parameter as close to zero since it is more likely to happen. Also, by applying NZR to the partially extracted parameters, we can assure that the absolute values of the parameters in the real model were higher than the absolute value of the parameters after reconstruction:

% |wnl| < |wl|

% This equation shows that if a parameter has a high absolute value after the reconstruction, it also has a high absolute value in the real DNN model. To reconstruct the un-extracted bits (bql=X), NZR first needs to know the sign bit of the parameter to reconstruct them as close to zero. If the parameter is positive, all of the un-extracted bits in that parameter will be assigned to zero. If the parameter is negative, all of them will be assigned to one. However, in some parameters, the sign bit is also unextracted. In this case, we consider the sign bit once positive and once negative and reconstruct the other unknown bits to get a near-zero weight wn+ , wn-. Then we compare wn+ and wn- to find in which case the absolute value of the parameter will be smaller, and we consider the smaller one to be the reconstructed weight. 

% \subsection{filter-wise L2-norm ranking (FL2R)}
% Performing bit-flip over hundreds of millions of weight bits in a DNN needs a tremendous amount of time. Therefore we need to prioritize each weight bit and only consider flipping the most sensitive weights (specifically sensitive bits) to create an accuracy drop. Previous works use each parameter's gradient (either computed via real or distilled data) to estimate its vulnerability. However, This approach is not applicable in a black box situation where there is no access to the dataset, and the parameters are not fully extracted to produce distilled data. In this work, we use a magnitude-based method to estimate the importance of the weight parameters in filter format. Then we try to find the most vulnerable parameter of the important weight filters and then flip their Most Significant Bit (MSB), their sign bit.

% Generally, in Deep Convolutional Neural Networks, the filters with higher l2-norm (lp-norm in general) lead to higher activation values in their corresponding output feature maps. Higher activation values will lead to a higher numerical impact on the final prediction of deep CNN models. In terms of this understanding, filters with a higher L2-norm have a higher importance in the model's functionality. Figure 2(a) illustrates the distribution of filters’ l2-norm value for each convolutional layer in a VGG-16 network trained on the CIFAR-10 dataset, where the distribution varies significantly across layers. There is limited number of filters with high l2-norm. Therefore, disrupting filters with a high L2-norm will be less time consuming, more effective and can reduce the model accuracy significantly.

% One of the most effective ways to neutralize and disrupt a filter's functionality is to decrease its l2-norm as much as possible. In other words, we need to perturb the parameter with the highest absolute value in the weight filter to make its absolute value close to zero. In order to make a parameter with a relatively high absolute value close to zero, we attack its most significant bit (sign bit). Suppose the weights in layer l are quantized in Nq bits. Changing the sign bit (b[nq -1]) will cause a $2^{nq-1}$ unit shift. Therefore The parameters with absolute values of $[2^{nq-1}-1 , 2^{nq-1} - 2^{nq-3}]$ will be changed to $[0 , 2^{nq-3}]$, which is the closest we can get by flipping only one bit in the memory.

% **injaro ye dor dige bas bekhoonam fek konam bad goftam**








%  \pagebreak
%  \pagebreak
% \section{TEST}

% \subsection{Attack Assumption }
% \begin{itemize}
%     \item Q0 past assumption?
%     \item Q1 our assumption?

% The attacker targets on ex-filtrating internal information (i.e., model weights) from deep learning systems by exploiting the underlying hardware fault vulnerabilities in modern computing systems. The attacker can control a user-space un-privileged process that runs on the same machine as the victim DNN service. We assume that the deep learning system is deployed on a resource-sharing environment to offer ML inference service. Such application paradigm is becoming popular due to the prevalence of machine-learning-as-a-service (MLaaS) platforms [55]. Our proposed framework manifest as a semiblack box attack where the adversary does not have any prior knowledge of the model weights. However, the attacker is aware of some key model architecture information, including model topology and layer sizes. We note that such an assumption is legitimate, as prior works demonstrate many practical ways to extract model architecture information through various side channel exploitation (e.g., through caches [5], memory bus [27] and EM [39]).

% Our attack mainly utilizes double-side rowhammer since fault occurrence in such setup exhibits stable data dependency. We assume that proper confinement mechanism is put in place to disallow direct access of data across processes. We further assume that the operating system and the hypervisor are benign and appropriate kernel-space protection mechanism are deployed to avoid direct tampering of kernel structures [57].

% We do not assume having any access to
% dataset.


% We assume that the attacker has only access to 80\% of parameters through side channel and row hammer attack. This assumption is legitimate based on previous works(deep steal).


%     \item Q2 applicability of black box attack
%     \item Q3: floating point? or quantization
% \end{itemize}



% \subsection{how to find DNN architecture?}
% \begin{itemize}
%     \item Q1: side channel attack
% \end{itemize}


% \subsection{partial parameter information reconstruction}
% \begin{itemize}
%     \item Q0: how to find some of the parameters? Ram-bleed (hammer-leak)
%     \item Q1: \textbf{why we can not use deep steal to attack the model and flip all the bits?}
%     \item Q2: why we can not retrieve full parameter information
% \end{itemize}
% Q1:The second challenge lies in developing an efficient rowham-mer attack that could successfully flip multiple bits within a reasonable exploitation window. We note that even with a very small number of bits to flip, the exploitation can still be unreasonably long. In fact, Gruss et al. have recently shown that a single bit flip in the victim’s memory can take a few days to accomplish [14]. As the disturbance errors in DRAM are transient, shortening the exploitation window for multi-bit flips is critical since the flipped bits generally do not persist after a memory reset or system reboot. Therefore it is legitimate to use deep steal as a preprocessing step to steal model parameters in advance and flips the bits after that. Note that deep steal takes Days to compute weights but performing 20 bit flips can be done in order of 1 minute.

% \subsection{Probabilistic weight reconstruction}
% \begin{itemize}
%     \item Q0: we use multivariate Bernoulli distribution and calculate $\rho(B_{unknown}|B_{known})$
%     \item Q1: \textbf{why does this method work?}
% \end{itemize}

% \subsection{Bit ranking}




% \begin{itemize}
%     \item Q0: why most significant bit?
%     \item Q1: \textbf{why we rank by absolute value?}
%     Filter selection. We use the Lp-norm to evaluate the importance of each filter as Eq. (2). In general, the convolutional results of the filter with the smaller Lp-norm lead to relatively lower activation values; and thus have a less numerical im- pact on the final prediction of deep CNN models. In term of this understanding, such filters of small Lp-norm will be given high priority of being pruned than those of higher Lp- norm.


%     ye chizi ham mishe emtehan kard inke berim filterayi ke miangine vaznashoon balast ro peyda konim va oonaro flip konim be soorate kashki.
%     \item Q1.25: l1-norm or l2-norm?
%     \item Q2: why only convolution layers?
%     \item Q3: why we flip only one direction in each filter?
% \end{itemize}

% \subsection{bit flip attack}
% \begin{itemize}
%     \item Q0: how to flip bits? row hammer
%     \item Q1: can we flip more than one bit per page?
% \end{itemize}






